Towards Monocular Shape from Refraction

Refraction is a common physical phenomenon and has long been researched in computer vision. Objects imaged through a refractive object appear distorted in the image as a function of the shape of the interface between the media. This hinders many computer vision applications, but can be utilized for obtaining the geometry of the refractive interface. Previous approaches for refractive surface recovery largely relied on various priors or additional information like multiple images of the analyzed surface. In contrast, we claim that a simple energy function based on Snell's law enables the reconstruction of an arbitrary refractive surface geometry using just a single image and known background texture and geometry. In the case of a single point, Snell's law has two degrees of freedom, therefore to estimate a surface depth, we need additional information. We show that solving for an entire surface at once introduces implicit parameter-free spatial regularization and yields convincing results when an intelligent initial guess is provided. We demonstrate our approach through simulations and real-world experiments, where the reconstruction shows encouraging results in the single-frame monocular setting.

==> local_figures/experiment_waves_quant.tex <==
\begin{figure}[!]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cccc}
         \multicolumn{2}{c}{\benchmarkname{wave1}} & \multicolumn{2}{c}{\benchmarkname{wave2}} \\
         \RMSE{} & \MAE{} [$^\circ$] & \RMSE{} & \MAE{} [$^\circ$]\\
         \includegraphics[width=0.25\linewidth]{local_images/experiments/wave1/wave1-RMSE-crop} & \includegraphics[width=0.25\linewidth]{local_images/experiments/wave1/wave1-MAE-crop} &         \includegraphics[width=0.25\linewidth]{local_images/experiments/wave2/wave2-RMSE-crop} & \includegraphics[width=0.25\linewidth]{local_images/experiments/wave2/wave2-MAE-crop} \\
    \end{tabular}}
    \caption{$\RMSE{}$ (left column) and $\MAE{}$ (right column) of the benchmark functions, \benchmarkname{wave1} [top] and \benchmarkname{wave2} [bottom]. 
    % 
    Each surface was rendered once with a flat background ($\zflat$, solid lines) and a curved surface ($\zfunc{}$, crosses). 
    %
    The complexity of the background surface has only very little effect on the quality of the solution, but the surface curvature has a strong effect on the initial guess \ref{sect:init}.
    % 
    %estimated surfaces because both functions manifest similar error regardless if we use the flat ($\zflat$) surface (solid line) or the $\zfunc{}$ function (crosses). 
    % 
    %The method is, however, sensitive to initialisation and when an initial surface depth is incorrect, the quality is reduced.  
    }
    \label{fig:experiment_waves_quant}
\end{figure}

==> local_figures/proof.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{local_images/proof/proof.pdf}
    \caption{Empirical proof of correctness of our energy function (\eq{eq:optim:energy}). 
    % 
    We performed an experiment where we used a ground truth surface from~\eq{eq:exp:wave1} and ran a series of optimizations, each one initialized by a plane which was gradually moved from the observer to the background.
    % 
    %
    For each experiment, the scatter plot shows the energy of both the initial guess $\dev{0}$ (red crosses) and the local minimum $\devh{i}$ (blue circles) as a function of their $\MSE{}$ from the ground truth $\devgt{}$.  The black dashed line represents the energy of our solution (the global minimum) which is very close to $0$.  
    % 
    %For better visibility, we show $\log{}$ values of both axes. 
    }
    \label{fig:optim:proof}
\end{figure}

% \begin{figure}[t]
%    \centering
%    \includegraphics[width=1.0\linewidth]{local_images/proof/proof.pdf}
%    \caption{Empirical proof of correctness of our energy in~\eq{eq:optim:energy} based on~\eq{eq:optim:dist}.
%    % 
%    We performed a synthetic experiment where we generated a $\Ngt{}$ ground truth surfaces $\devgt{}$ around $2$ and gradually disturbed ($j$, see \eq{eq:proof:devgt}) its value with a Gaussian noise and $\Nh{}$ hypothesized surfaces $\devh{}$ gradually disturbed ($i$, see \eq{eq:proof:devh}) from ground truth surface with Gaussian noise and evaluated our energy.   
%    %
%    Figure shows empirical evidence that our energy gets close to 0  as the hypothesised surface $\devh{}$ is approaching to ground truth $\devgt{}$.
%    % 
%    We used $\log{}$ of original energy $\len{}$ and clamped lower values to 0 on $z$-axis for better visibility.
%    }
%    \label{fig:optim:proof}
% \end{figure}
% \end

==> tex/old-proofs.tex <==
\paragraph{Theorem} The light path $\Xr{} + t\s{}=\de{} \LOS{} + t\s{}$ and is intersecting with background point $\Xr{}$ is the only solution correct solution. 

\paragraph{Proof} 
%
We prove it by Fermat's principle. 
%
Fermat principle states that light a path taken by a ray of light in traveling between two points in stationary time. % for now taken from https://www.britannica.com/science/Fermats-principle
We have to show that there is no other light path whose travel time is stationary and we prove it by contradiction. 
% 
We know that Snell's law is derived from Fermat's principle. We further know form the assumption that $\Xr{} + t\s{}=\de{} \LOS{} + t\s{}$ follows Snell's law so the Fermat's principle. 
% 
Consider an arbitrary point $\de{}'\neq \de{}$ on $\LOS{}$ which is also intersecting with the same background point $\Xb{}$ where $\s{}'$ which is a vector between $\Xr{}'=\de{}'\LOS{}$ and $\Xb{}$. 
% 

\begin{equation}
    \begin{array}{c}
    \frac{\|\Xr{}'\|}{v_1} + \frac{t'\s{}'}{v_2}
    \end{array}
\end{equation}
How to prove this?
$\qed{}$

%
% Now, we want to show the relation between surface points and normals. We assumed that the direction of refraction $\s{}$ is known and following Snell's law, but $\s{}$ in \eq{eq:bg:snell} depends on the normal $\n{}$ which requires surface derivative. 
% 
% In the following theorem, we show that the energy is zero iff the depths of two adjacent surface points are obeying Snell's law and is a global optimum. 

%
% The theorem needs clearly defined assumptions and assertions, and the
% assertions need to follow only from the assumptions, and not anything implicit
% in the surrounding text.
% Lets' write them down here before putting it in a theorem. I'll write what I
% understood from the text (which was not really clear to me, so please
% correct as necessary):
%
% ASSUMPTIONS:
% a) fixed l_1 and l_2 are given
% b) fixed d_1 and d_2 are given (which defines X_1 and X_2)
% c) fixed (but arbitrary) n_1 and n_2 are given,
% d) B is given
% e) E( X_1, s_1, B ) = 0 and E( X_2, s_2, B ) = 0
%
% ASSERTIONS:
% A) Snell's law is satisfied, i.e. s_i = snell( l_1, n_1, \mu )
% B) d_1 and d_2 as well as n_1, n_2 are unique.
% C) Global optimality holds.
%
% Comments / problems:
% 1) I do not know where you get s_1 and s_2 from. You can compute them from
%   (c) using Snell's law, then (A) is obviously true. However, then the
%   energy is only zero if the normals are actually the true normals.
%   Is this an additional assumption which is missing?
% 2) (C) is obvious, since E>=0, then you have a global optimum if (e) holds
% 3) I can't follow the arguments why (B) should hold. There must be implicit
%   assumptions or a misunderstanding, since there is no reason for this
%   in the current setting.
% 4} The two rays are not linked in the assumptions at all, so I have no
%   idea why there even are two. This is why I also believe there is some
%   implicit assumption missing.
% Antonin: 1) s_1,s_2 are based on true normals n_1,n_2, that's why I assume, I want to prove that there is only one pair  of d_1,d_2. I added this into proof.
% 2) I only wanted to mention it to make it clear that this is unique
% 3) X_1,X_2 are calculated from d_1,d_2, any combination would lead to a unique pair X_1,X_2 thus n_1,n_2, so there is no d_1',d_2' which would lead to the same normals n_1,n_2 when at least one of the points is different from d_1,d_2 (in a simple way, depth to normals is injective mapping)
% 4) I forgot to mention, that these surface points must be infinitely close, this is good point, I hope that this statement would fix it
%
%
% I think I finally get what you are trying to show. 
% The following needs to go into the assumptions of the theorem then:
% (correct me if I'm wrong):
%
% We assume X_1 and X_2 are close, and the surface is approximated
% by it's tangent plane, which is determined by either of the normals.
%
% In this case, I can believe the uniqueness claim, but a reformulation
% would be required. The thing is that X_2 is already completely determined
% by the choice of X_1, as this already defines a fixed surface normal via
% Snells' law. You therefore get X_2 by computing the intersection of
% the resulting tangent plane with l_2.
%
% So, here's a possible sketch of a proof which would probably work,
% but it's direct and might be a bit messy:
%
% - Compute the required normal n_1 from Snell's Law given a fixed X_1
% - Compute X_2 from X_1, n_1 and l_2
% - Compute the projection B_2^\prime of X_2 onto the background plane
% - Show that the location depends on the choice of X_1.
% - Alternatively, if computing n_1 is too cumbersome, you can just
%   assume that you have computed one, and demonstrate that when you
%   change the location of X_1 infinitesimally, then there is
%   a change in B_2^\prime. Formulas might also become simpler if you
%   assume parallel rays l_1, l_2, i.e. l_1=l_2=l.
%
% This would be the required contradiction, since B_2 is fixed from
% the choice of l_2, i.e. if you have found a solution, it must be
% the only one.
%
% 
% Remaining problems:
% - uniqueness of the solution is good, but not sufficient, what you
%   should show is that your proposed scheme converges. This is not
%   guaranteed as far as I can see, since you iterate a global optimization
%   step with a full reinitialization of the normals (which in theory
%   might fluctuate around wildly).
% Antonin: This might really be a problem to prove, but in case that points are infinitesimally close to each other? Or the normals are "fixed" and "known". Another thing is that I am not proving convergence of the optimisation, but only that the energy in Eq.(4) is 0 
%
% B: This is not a problem for this theorem, but for the overall paper. Even if you show that a unique solution to
%    the problem exists, it is not clear that your method computes it - you neither have shown that the
%    method converges at all, nor that it converges to a solution where E=0.
%    However, your experiments indicate that this is experimentally correct, and there are many
%    papers around which do not deliver such a proof. I would not try to do this for the
%    submission deadline, but it should be mentioned somewhere in the paper.
% A: You mean a proof of E=0, or proof of convergence? The point of the proof is to convince reader that $E=0$ for a correct solution. 




%
% The theorem needs clearly defined assumptions and assertions, and the
% assertions need to follow only from the assumptions, and not anything implicit
% in the surrounding text.
% Lets' write them down here before putting it in a theorem. I'll write what I
% understood from the text of the theorem:
% ASSUMPTIONS:
% a) a fixed l is given
% b) a fixed s is given (which then implicity defines n)
% c) B is given
% ASSERTIONS:
% If (a)-(c) hold, then there is only one d such that
% the resulting ray passes through B.
%
% The problem: This is not true, because it only holds in 2D. In 3D, there
% generally is no d such that the ray passes through B, since l, s
% and B given in (a)-(c) are in general not coplanar.
% Thus, there are assumptions missing. Which are they?
% 
% Antonin: I think they are co-planar: 
% s and l are forming a plane and since s is based on the snell's law, so s and l make a plane where is B even in 3D, 
% the point which should probably make the proof clearer is that s is related to B
\iffalse
\vspace{-1.0em}
\paragraph{Theorem (1)} For known Snell's direction $\s{}$ and fixed $\LOS{}$, $\Xb{}$ there exists only one distance $\de{}$ which defines $\Xr{}$ though which light path goes and intersects with $\Xb{}$.

\noindent \textbf{Proof of Theorem (1)} With fixed $\s{}$ and $\LOS{}$, we move the vector $\s{}$ along $\LOS{}$, until line from $\de{}\LOS{}$ in direction $\s{}$ intersects with $\Xb{}$. See~\fig{fig:bg:schema} [right] for schematic illustration of the proof. 
% 
There is only one such point, which is at $\de{}$.~$\qed{}$

\vspace{-1.0em}
\paragraph{Corollary (1)} When a light path is intersecting with its corresponding background point $\Xb{}$ then $\len{} = 0$. 
%

\noindent \textbf{Proof of Corollary (1)} The point goes through $\Xb{}$ thus from~\eq{eq:optim:dist}, $\len{}$ must be 0.~$\qed{}$
\fi

\iffalse
\paragraph{Theorem} Consider two surface points $\Xr{1},\Xr{2}$ defined by their fixed $\LOS{1},\LOS{2}$ and $\de{1},\de{2}$ which are following Snell's law with IOR $\mu$ and intersect with their corresponding background points $\Xb{1},\Xb{2}$, there is no other combination of $\de{1}'=\de{1}+\epsilon_1,\de{2}'=\de{2}+\epsilon_2$ s.t. $\epsilon_1>0$ or $\epsilon_2>0$ which would for a fixed $\LOS{1},\LOS{2}$ and $\Xb{1},\Xb{2}$ form a pair of light paths and intersect with $\Xb{1},\Xb{2}$. 

\paragraph{Proof}
From the assumption, the light paths defined by $\de{1},\de{2}$ intersect with their background points. We would like to show that this light path is for a fixed $\LOS{1},\LOS{2}$ and $\Xb{1},\Xb{2}$ unique. 
%
\fig{fig:bg:schema} [right] schematically shows our situation. 
%
We prove it by contradiction. 
%

Consider $\de{1}'=\de{1} + \epsilon$, s.t. $\epsilon\neq 0$, thus $\Xr{1}'=(\de{1}+\epsilon)\LOS{1}=\de{1}\LOS{1}+\epsilon\LOS{1}$. 
% 
We obtain a pair of points $\Xr{1}',\Xr{2}$. Since $\Xr{1}'\neq \Xr{1}$, both normals $\n{1}',\n{2}'$ are changed.
%
Angle subtended by $\LOS{}$ and $\n{}$ is in range $(\pi/2,\pi/2)$ and Snell's law is strictly monotonous and bijective in this range and following inequality holds
\begin{equation}
    \s{}(\LOS{},\n{},\mu)\neq \s{}(\LOS{},\n{}',\mu)\;\;\ \text{ where } \n{}\cdot\LOS{}\neq\n{}'\cdot{}\LOS{}.
    \label{eq:optim:sb}
\end{equation}
%

From \eq{eq:optim:sb} implies that we obtain a new pair of $\s{1}',\s{2}'$ where $\s{1}'\neq \s{1},\s{2}'\neq \s{2}$ and a new pair of of light paths
$$
    \begin{array}{ccc}
         \Xr{1}'+t_1\s{1}' & \text{ and } & \Xr{2} + t_2\s{2}'.
    \end{array}
$$

From contradiction assumption both points $\Xr{1}',\Xr{2}$ form light paths which intersect with $\Xb{1},\Xb{2}$. 
% 
We now take the opposite path where we go from from $\Xb{1},\Xb{2}$ along $\LOS{1}'=-\s{1}',\LOS{2}'=-\s{2}'$, \ie{}
$$
    \begin{array}{ccc}
         \Xb{1}+t_1'\LOS{1}' & \text{ and } & \Xb{2}+t_2'\LOS{2}' ,
    \end{array}
$$

\noindent where $\LOS{1}',\LOS{2}'$ are a "reverse" line of sight from $\Xb{1},\Xb{2}$ through $\Xr{1}',\Xr{2}$. 
% 
Since we know $\n{1}',\n{2}'$ and $\LOS{1}',\LOS{2}'$, we can calculate the "reverse" refraction 
$$
\begin{array}{ccc}
\s{1}''=\s{}(\LOS{1}',-\n{1}',\mu^{-1}) & \text{ and } \s{2}''=\s{}(\LOS{2}',-\n{2}',\mu^{-1})
\end{array}
$$
\noindent which must have the same angle as $-\LOS{1},-\LOS{2}$. From bijection of Snell's law in \eq{eq:optim:sb} and since at least one $\LOS{1}'\neq \s{1}$ or $\LOS{2}'\neq\s{2}$, it implies that going reversely does not go along their original lines of sight, \ie{} $\s{1}''\cdot{}(-\LOS{1}),\s{2}''\cdot{}(-\LOS{2})\neq 1$. We prove that this there is no other combination of depths $\de{1}',\de{2}$  which can intersect with the background point $\Xb{1},\Xb{2}$. $\qed$

\paragraph{Proof 2 (more general)} % 
From the assumption, the light paths defined by $\de{1},\de{2}$ intersect with their background points. We would like to show that this light path is for a fixed $\LOS{1},\LOS{2}$ and $\Xb{1},\Xb{2}$ unique. 
%
\fig{fig:bg:schema} [right] schematically shows our situation. 
%
We prove it by contradiction. 
%

Consider $\de{1}'=\de{1} + \epsilon$, s.t. $\epsilon_1\neq 0$, thus $\Xr{1}'=(\de{1}+\epsilon)\LOS{1}=\de{1}\LOS{1}+\epsilon\LOS{1}$ and  $\de{2}'=\de{2} + \epsilon$, s.t. $\epsilon_2\neq 0$, thus $\Xr{2}'=(\de{2}+\epsilon)\LOS{2}=\de{2}\LOS{2}+\epsilon\LOS{2}$. 
% 
We obtain a pair of points $\Xr{1}',\Xr{2}'$. Since $\Xr{1}'\neq \Xr{1},\Xr{2}'\neq \Xr{2}$, both normals $\n{1}',\n{2}'$ are changed\footnote{there is a special case of flat surface, I will get to it eventually later! but normals will be same if you change depth of two flat points identically }.
%
Angle subtended by $\LOS{}$ and $\n{}$ is in range $(\pi/2,\pi/2)$ and Snell's law is strictly monotonous and bijective in this range and following inequality holds
\begin{equation}
    \s{}(\LOS{},\n{},\mu)\neq \s{}(\LOS{},\n{}',\mu)\;\;\ \text{ where } \n{}\cdot\LOS{}\neq\n{}'\cdot{}\LOS{}.
    \label{eq:optim:sb}
\end{equation}
%

From \eq{eq:optim:sb} implies that we obtain a new pair of $\s{1}',\s{2}'$ where $\s{1}'\neq \s{1},\s{2}'\neq \s{2}$ and a new pair of of light paths
$$
    \begin{array}{ccc}
         \Xr{1}'+t_1\s{1}' & \text{ and } & \Xr{2}' + t_2\s{2}'.
    \end{array}
$$

From contradiction assumption both points $\Xr{1}',\Xr{2}'$ form light paths which intersect with $\Xb{1},\Xb{2}$. 
% 
We now take the opposite path where we go from from $\Xb{1},\Xb{2}$ along $\LOS{1}'=-\s{1}',\LOS{2}'=-\s{2}'$, \ie{}
$$
    \begin{array}{ccc}
         \Xb{1}+t_1'\LOS{1}' & \text{ and } & \Xb{2}+t_2'\LOS{2}' ,
    \end{array}
$$

\noindent where $\LOS{1}',\LOS{2}'$ are a "reverse" line of sight from $\Xb{1},\Xb{2}$ through $\Xr{1}',\Xr{2}'$. 
% 
Since we know $\n{1}',\n{2}'$ and $\LOS{1}',\LOS{2}'$, we can calculate the "reverse" refraction 
$$
\begin{array}{ccc}
\s{1}''=\s{}(\LOS{1}',-\n{1}',\mu^{-1}) & \text{ and } \s{2}''=\s{}(\LOS{2}',-\n{2}',\mu^{-1})
\end{array}
$$
\noindent which must have the same angle as $-\LOS{1},-\LOS{2}$. From bijection of Snell's law in \eq{eq:optim:sb} and since at least one $\LOS{1}'\neq \s{1}$ or $\LOS{2}'\neq\s{2}$, it implies that going reversely does not go along their original lines of sight, \ie{} $\s{1}''\cdot{}(-\LOS{1}),\s{2}''\cdot{}(-\LOS{2})\neq 1$. We prove that this there is no other light path which can intersect with the background point $\Xb{1},\Xb{2}$. $\qed$
\fi

\iffalse
\paragraph{Theorem} Two light paths which are obeying Snell's law defined by two adjacent points~\mbox{$\Xr{1}=\de{1}\LOS{1}, \Xr{2}=\de{2}\LOS{2}$} intersect with their respective background points $\Xb{1},\Xb{2}$ are unique and globally optimal iff \mbox{$\len{1},\len{2}=0$}.

\paragraph{Proof} 
We show that there is only one pair of points $\Xr{1},\Xr{2}$ with their unique normals $\n{1},\n{2}$ (calculated from these two points) and $\s{1},\s{2}$ (calculated from the normals and lines of sight) which follow Snell's law and intersect their respective background points $\Xb{1},\Xb{2}$ and thus $\len{1},\len{2} = 0$.
%
We prove it by contradiction.
%

Assume that there is another a pair of surface points $\Xr{1}'=\de{1}'\LOS{1},\Xr{2}'=\de{2}'\LOS{2}$ on the same $\LOS{1},\LOS{2}$ where at least one $\de{1}',\de{2}'$ is different from $\de{1},\de{2}$ but from the contradiction still intersect with their background points. 
%
For such pairs of points, we obtain a pair of normals $\n{1}',\n{2}'$. 
% 

Angle subtended by $\LOS{}$ and $\n{}$ is in $(-\pi/2,\pi/2)$ and Snell's function is bijective in this range. 
%
The aforementioned bijection implies that for fixed $\LOS{1},\LOS{2}$, points $\Xr{1}',\Xr{2}'$ and their normals $\n{1}',\n{2}'$ form another unique pair of light paths.
%
\footnote{Note that even in case that $\Xr{1},\Xr{2}$ are on flat surface and normals are same light paths are sill different since $\de{}$ are still different.}
%
where at least one light path cannot intersect with its background point since its normal create a different light path (bijection) and is $\len{}>0$ thus such pair does not exist
%
Since $\len{} \geq 0$ and $\len{}$ is $0$ only at the correct solution, this optimum is unique and global.~$\qed{}$

Theorem (1) and Corollary (1) state that there is a path that yields Snell's law and is $\len{} = 0$ and in Theorem (2) we show that there is only a single pair of paths which are following Snell's law. 
% 
We need at least two points to be able to determine normals and render light paths. Theorem (2) can be easily extended to multiple points, but at least two points are needed and each path uniquely defines the value of $\len{}$ in a combination of its neighbours and they all are following Snell's law only when their energies are zero.
%
Note that $\len{}$ itself is not bijective. There might be other local minima, but $\len{}=0$ is only one. 
\fi

==> tex/proof.tex <==
\input{local_figures/proof}

% \input{tex/old-proofs}

We want to show empirically that the correct solution is a global minimum of our energy in~\eq{eq:optim:energy}.
%We show empirically, that when we optimise for~\eq{eq:optim:energy} we never obtain a solution that has lower or similar energy as ground truth and is away from our correct solution at the same time. 
% 
To do this we created the following experiment. We considered a canonical calibration, a flat background surface at $z_B=2.5$ and a ground truth surface defined by $\devgt{}=z_{\text{wave1}}(x,y,0)$  (\eq{eq:exp:wave1}). As it is not possible to calculate the energy for all possible surfaces, we decided to calculate the energy of local minima of the function.  To find the local minima, we run a series of $\Nh{}=100$ optimizations, each optimization is initialized with a plane at $\dev{0}(j)$ which is gradually moved from the camera towards the background $z_B$  
\begin{equation}
\dev{0}(j) = z_B\frac{j}{\Nh{}}~~, ~~ j\in\{1,\dots \Nh{}\} \;\;.
\label{eq:proof:dev0}
\end{equation}
Every initial solution $\dev{0}(j)$ yields a different surface solution $\devh{}(j)$ which is significantly modified from the initial guess during optimization. We plug each of the solutions $\devh{}(j)$ into \eq{eq:optim:energy} to calculate its energy.
%
 

\fig{fig:optim:proof} depicts the scatter plot of the resulting energies as a function of the distance of the local minima from the global one. 
%
For different initializations, that are sufficiently far from the ground truth, the optimization often got trapped in a local minimum. As seen in \fig{fig:optim:proof}, in all solutions that are far from the ground truth the energy is much higher than the energy of the ground truth, indicating the ground truth is a global minimum. 
% 
%This demonstrates that in a large number of samples ($\Nh{}=100$), the optimisation never converges to another solution whose energy is similar to the ground truth energy and is still not correct.


\iffalse
\input{local_figures/proof}

We empirically show, that when we optimize for \eq{eq:optim:energy} we get as close as possible to correct surface geometry. 
%
We conducted the following synthetic experiment. For a canonical calibration matrix, we generate $\Ngt{}$ random surfaces as our ground truth surfaces and gradually fluctuate with Gaussian noise as 
\begin{equation}
\begin{array}{ccc}
\devgt{}(j) = 2 + \frac{j}{N_{\text{gt}}}\noise{0.1} & \text{ for } & j\in\{0,\dots \Ngt{}\}
\end{array}
\label{eq:proof:devgt}
\end{equation} 
%

Note that growing $j$ adds more noise to $\devgt{}$. 
%
We further generated a hypothesized surface $\devh{}$ which we gradually fluctuate with Gaussian noise as 
\begin{equation}
\begin{array}{ccc}
\devh{}(j) = \devgt{} + \frac{i}{\Nh{}}\noise{0.1}  & \text{ for } & i\in\{0,\dots \Nh{}\}
\end{array}
\label{eq:proof:devh}
\end{equation}

Gradually increasing the value of $i$ moves $\devh{}$ away from the ground truth surface $\devgt{}$. Evaluation of energy~\eq{eq:optim:dist} on $\devgt{}$ and $\devh{}$ is shown in~\fig{fig:optim:proof}.
% 
The plot shows that for increasing values of noise ($i$), the energy grows as the hypothesized depth $\devh{}$ moves away from the correct estimate. 
%
There is a noticeable step at $i=0$ where a hypothesized $\devh{}$ is identical with $\devgt{}$ where energy steeply converges to zero.
%
Furthermore, when we increase $j$, we disturb ground truth and add more non-smoothness which creates estimation more challenging.
%
It is important to show that energy still gets lower even though the ground truth surface $\devgt{}$ is strongly disturbed by Gaussian noise since it can affect the accuracy of calculation of the normals.
%
The script for the empirical proof is part of supplementary material.

\fi
